Search@Home: A Commercial Off-the-Shelf Environment for Investigating Optimization Problems

Search heuristics, particularly those that are evaluation-driven (e.g., evolutionary computation), are often performed in simulation, enabling exploration of large solution spaces. Yet simulation may not truly replicate real-world conditions. However, search heuristics have been proven to be successful when executed in real-world constrained environments that limit searching ability even with broad solution spaces. Moreover, searching in situ provides the added benefit of exposing the search heuristic to the exact conditions and uncertainties that the deployed application will face. Software engineering problems can benefit from in situ search via instantiation and analysis in real-world environments. This paper introduces Search@Home, an environment comprising heterogeneous commercial off-the-shelf devices enabling rapid prototyping of optimization strategies for real-world problems.

==> sections/04-results.tex <==
This section describes our experimental setup and results for two applications deployed to \ToolName: a string search algorithm and a continuously-running load-balanced web server.

For each case study, we performed $25$ experimental replicates (i.e., each replicate is a repeatably-seeded evaluation) to ensure statistical significance.  For each statistical evaluation in this section, we use the Wilcoxon-Mann-Whitney U-test with a significance level of $0.001$ (i.e., $p < 0.001$).  Each case study was also compared to random search to demonstrate the GA's effectiveness, as specified by Arcuri~\etal{}~\cite{arcuri.2011}.

\subsection{String Search}

The purpose of using a relatively simplistic search application is to essentially ``prove out'' the feasibility of running an optimization procedure on a constrained device.  As such, the search algorithm was configured as specified in Section~\ref{sec:string}.  Each experimental replicate ID (i.e., [$1$, $25$]) was used as an input to seeding the random function for repeatability.  For this particular experiment, we are interested in the amount of time required before convergence to the expected solution and the number of generations necessary to reach that value, as the number of generations is set very high to ensure convergence.  We compare these values to those performed on a current-generation laptop (Intel Core i7 quad-core 2.8GHz 64-bit processor, 16GB RAM, 1TB hard drive space).  The microcomputers used for this experiment were a Raspberry Pi 3B with an ARM quad-core 1.2GHz 64-bit processor, 1GB of RAM and 16GB of hard drive space and a Raspberry Pi 4B with an ARM quad-core 1.5GHz 64-bit processor, 4GB of RAM, and 16GB of hard drive space.  To focus on execution time, we intentionally did not introduce parallelism, however such a procedure can be used on a microcomputer.\footnote{Both Raspberry Pis have 4 processor cores and could leverage Python's \texttt{multiprocessing} package, for example.}

\vspace{0.2in}

\noindent \textbf{Experimental Results}  We define our null hypothesis $H1_0$ to be ``there is no significant difference in execution times between experiments performed on a laptop and a microcomputer,'' where the alternate hypothesis $H1_1$ states that ``there is a significant difference in execution times between experiments performed on a laptop and a microcomputer.'' 

To demonstrate this hypothesis, Figure~\ref{fig:stringsearch}(a) compares the number of generations required for the algorithm to converge and Figure~\ref{fig:stringsearch}(b) compares the amount of time (seconds) required to reach convergence.  

\begin{figure}[htb!]%
    \centering
    \subfloat[Number of generations.]{{\includegraphics[width=5.5cm]{figures/string-search-gens.png}}} %\includegraphics[width=5cm]{img1} }}%
    \qquad
    \subfloat[Execution time.]{{\includegraphics[width=5.5cm]{figures/string-search-time.png}}} %\includegraphics[width=5cm]{img2} }}%
    
    \vspace{-0.10in}
    
    \caption{Comparison of string search results between laptop and microcomputer.}%
    \label{fig:stringsearch}%
\end{figure}

As can be seen from these figures, there exists no difference in the number of generations required to converge to the optimal solution.  However, a significant difference exists between the execution times required for convergence between the two devices ($p < 0.001$).  Moreover, each experimental replicate resulted in convergence.  These results are expected given the disparity in processing capability.  However, the Raspberry Pi was able to successfully execute optimization in all cases within a reasonable amount of time, proving feasibility of optimization on constrained devices and enabling acceptance of our alternate hypothesis $H1_1$.
%dispy of normal calculations in separate section?

\iffalse

\subsection{Load Balanced Web Application}

To demonstrate the feasibility of running search optimization \textit{in situ} within a constrained environment, we deployed the \texttt{HAProxy} load balancing software as described in Section~\ref{sec:haproxy}.  Nodes \texttt{raspberrypi01} and \texttt{raspberrypi02} each served a lightweight NodeJS-driven website that only described the page's origin (e.g., \textit{Hello from 192.168.1.102}, where $192.168.1.102$ was the IP address of \texttt{raspberrypi02}).\footnote{Given that we are mainly interested in downtime and HTTP response codes, a complex website is not necessary.}  Each member of the population was evaluated sequentially, given that optimization was being performed online (i.e., live evaluation precluded the use of parallelization).  For each evaluation, the \texttt{HAProxy} service was restarted to ensure that all collected metrics were reset and a five second delay was added to ensure \texttt{HAProxy} had properly initialized.  The default logging behavior for \texttt{HAProxy} was disabled as well as the number of logs generated quickly outpaces the $16$GB microSD card on the Raspberry Pi.

To simulate load, \texttt{Bombardier} was executed on the \texttt{netbook} and targeted the frontend (\texttt{pi-master}).  To ensure continuous load testing, \texttt{Bombardier} was executed for the entirety of each search procedure.  For this paper, we configured \texttt{Bombardier} to use $500$ concurrent connections using HTTP \texttt{GET} requests, ensuring that \texttt{HAProxy} could effectively distribute traffic to nodes \texttt{raspberrypi01} and \texttt{raspberrypi02}.

\vspace{0.2in}

\noindent \textbf{\textit{In situ} search}: We first explored the use of a GA in a constrained environment.  For this experiment, we define our null hypothesis $H2_0$ to state that ``there is no difference in network performance between randomly-generated load balancer configurations to those discovered by an online search procedure.''  Our alternate hypothesis $H2_1$ states that ``there is a difference in network performance between randomly-generated load balancer configurations to those discovered by an online search procedure.''  To test these hypotheses, we executed a GA and random search within \ToolName, where an equivalent number of evaluations was performed for each experimental replicate (i.e., $100$ evaluations per replicate).  Both \ToolName, random search, and the GA were configured as specified in Section~\ref{sec:haproxy}.  

Figure~\ref{} presents the fitness scores between configurations generated by the GA and those generated by random search.  

\begin{figure}
    \centering
    \includegraphics[width=3.2in]{figures/SSBSE20_HAProxy_Fitnesses}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

One issue that exists in performing search in a production environment is the possibility of catastrophic failure.  For our purposes this is not necessarily a problem, as the system is simply unavailable for the duration of the genome's active state (generally, when both \texttt{raspberrypi01} and \texttt{raspberrypi02} were both configured to be in a \texttt{DRAIN} state, meaning no servers were available).  However, for a system where uptime is a necessity then exploration in a sandboxed (i.e., duplicate of production environment) or symbiotic environment (i.e., live data from production transmitted to a simulation)~\cite{} may be more appropriate.

* Commonality in good genomes
* Average execution time

\vspace{0.2in}

\noindent \textbf{\textit{In situ} continuous search}: To further explore the benefits of \textit{in situ} online optimization, we applied the \texttt{(1+1)-ONLINE EA}~\cite{bredeche.2010} to \ToolName, where we reuse the genome, fitness functions, and mutation operator from the previous section.  For this experiment, we only use mutation to guide the search procedure.  Each active genome was evaluated for a period of $60$ seconds, where the poorer-performing genome was discarded after comparison.  To enable a reasonable comparison to the full genetic algorithm, we executed each experimental replicate for $214$ minutes, where $214$ minutes is the average time required to execute a full experimental replicate from the prior experiment.  The initial genome was randomly generated for each replicate.

For this experiment, ...
\fi

\subsection{Threats to Validity}  

This research has been a proof of concept to demonstrate the feasibility of extending the SBSE domain to real-world devices using COTS hardware.  As such, we have identified the following threats to validity.  One threat to validity lies in the selected hardware, as we focused on the Raspberry Pi platform, however other devices exist that may be more targeted towards the application domains (i.e., network appliances that strictly perform load balancing) and therefore be either more or less capable in terms of optimization feasibility.  Another threat to validity lies in the configuration of our search algorithms, as no tuning was performed on the evolutionary parameters.  Additionally, we also did not perform online search in a safety-critical domain, and as such, only report our results in domains that are not negatively impacted by a search procedure while executing.  We also limited our investigations to GAs for search, however there exist many other optimization algorithms in other domains (i.e., evolutionary, continuous, probabilistic, etc.), including multi-objective optimization~\cite{deb.2002}, novelty search~\cite{lehman.2004}, Bayesian optimization~\cite{shahriari.2015}, and Markov chains~\cite{calinescu.2010}.


%%% RERUN SEED 5 FOR GA

==> sections/05-related-work.tex <==
This section presents related work in online optimization and SBSE in constrained systems.

\subsection{In Situ Optimization}

symbiotic

sandboxed

\textit{In situ} optimization has been applied to wireless sensor network applications, where run-time reconfiguration models and programming models are used to enable optimization~\cite{taherkordi.2013}.  Fredericks~\etal{} combined evolutionary computation with continuous optimization and clustering methods to optimize support planning in self-adaptive systems~\cite{fredericks.2019.saso}.  \textit{In situ} optimization has also been applied to the software engineering domain.  Li~\etal{} studied the energy-efficiency of test suites in low power systems~\cite{li.2014}.

Continuous optimization is a common feature in other applications as well.  For instance, Wang and Boyd have applied an online optimization technique (a primal barrier method) to model-predictive control applications~\cite{wang.2009.cst}.  Mars and Hundt have combined static and dynamic optimization strategies to direct online reconfiguration based on scenarios~\cite{mars.2009}.  Optimization has also been applied online in a data-driven capacity, where uncertainty models can inform  decision making~\cite{bertsimas.2006}.

\subsection{Search-based Software Engineering in Constrained Systems}


